Few-Shot Classification in Unseen Domains by Episodic Meta-Learning Across Visual Domains

Few-shot classification aims to carry out classification given only few labeled examples for the categories of interest. Though several approaches have been proposed, most existing few-shot learning (FSL) models assume that base and novel classes are drawn from the same data domain. When it comes to recognizing novel-class data in an unseen domain, this becomes an even more challenging task of domain generalized few-shot classification. In this paper, we present a unique learning framework for domain-generalized few-shot classification, where base classes are from homogeneous multiple source domains, while novel classes to be recognized are from target domains which are not seen during training. By advancing meta-learning strategies, our learning framework exploits data across multiple source domains to capture domain-invariant features, with FSL ability introduced by metric-learning based mechanisms across support and query data. We conduct extensive experiments to verify the effectiveness of our proposed learning framework and show learning from small yet homogeneous source data is able to perform preferably against learning from large-scale one. Moreover, we provide insights into choices of backbone models for domain-generalized few-shot classification.

==> tables/table_2.tex <==
\begin{table*}[t]
    \caption[c]{Performance comparisons on Omniglot, Mini-ImageNet, and CUB using RelationNet as the backbone models. Note that Single Domain-S indicates the training of RelationNet with support and query sets always from the same domain S, and x-EML* denotes the training of our model using support and query sets sampled from the same domain in each episode. The averaged accuracy is reported along with the 95\% confidence interval. \label{table:2}}
    
    \resizebox{1.0\linewidth}{!}{
         \begin{tabular}{l|c|c|c|c|c|c}
         & \multicolumn{2}{c|}{Omniglot} & \multicolumn{2}{c|}{Mini-ImageNet} & \multicolumn{2}{c}{CUB} \\ \cline{2-7}
        \textbf{Method} & 1-shot & 5-shot & 1-shot & 5-shot & \multicolumn{1}{c|}{1-shot} & 5-shot \\ \cline{1-7}
        
        \textbf{Single Domain-S} & $51.15\pm0.96$ & $70.02\pm0.98$ & $24.93\pm0.50$  & $29.90\pm0.51$ & $24.72\pm0.44$ & $31.76\pm0.53$ \\
        \textbf{Single Domain-C} & $56.28\pm1.01$ & $73.36\pm0.94$ & $27.32\pm0.57$ & $33.00\pm0.59$ & $28.10\pm0.59$ & $32.66\pm0.57$\\
        \textbf{Single Domain-A} & $56.07\pm1.05$ & $61.02\pm0.97$ & $29.91\pm0.60$ & $34.91\pm0.60$ & $26.55\pm0.53$ & $31.90\pm0.53$\\ \hline
        \textbf{LFT \cite{tseng2020cross}} & $57.86\pm0.98$ & $\bf 79.17\pm0.86$ & $28.09\pm0.54$ & $35.95\pm0.55$ & $\bf 29.65\pm0.55$ & $35.68\pm0.59$ \\ \hline
        \textbf{x-EML*} & $56.11\pm1.01$ & $74.56\pm0.86$ & $29.25\pm0.57$ & $36.54\pm0.62$ & $28.36\pm0.60$ & $\bf 36.27\pm0.64$\\ \hline
        \textbf{x-EML (Ours)} & $\bf 58.12\pm0.94$ & $77.89\pm0.85$ & $\bf 30.90\pm0.64$ & $\bf 39.15\pm0.62$ & $27.30\pm0.52$ & $34.94\pm0.57$\\
        
        \end{tabular}
    }
\end{table*}

==> tables/table_4.tex <==
\begin{table*}[t]
    \centering
    \caption[c]{Effects of backbones with varying depths on domain-generalized few-shot classification. We consider ProtoNet as the backbone of our x-EML framework, and Conv-\(n\) indicates \(n\) ConvBlocks. Note that x-EML is trained on PACS in 3-way 5-shot settings, with results presented on PACS, Omniglot, mini-ImageNet, and CUB. It can be seen that, use of deeper backbones is not necessarily preferable for domain generalization due to possible overfitting of source domains. \label{table:4}}
    
    \resizebox{0.8\linewidth}{!}{
        \begin{tabular}{c|c|c|c|c}
         Depth & {PACS \(\to\) PACS} & Omniglot & Mini-ImageNet & CUB \\ \cline{1-5}
        Conv-2 & \(62.88\pm1.32\) & \(92.33\pm0.67\) & \(55.41\pm0.89\) & \(52.73\pm0.82\) \\
        Conv-3 & \(64.55\pm1.28\) & \(\bf 94.74\pm0.57\) & \(60.11\pm0.87\) & \(57.55\pm0.85\) \\
        Conv-4 & \(64.78\pm1.39\) & \(94.17\pm0.60\) & \(\bf 61.38\pm0.88\) & \(\bf 58.59\pm0.85\) \\
        Conv-5 & \(64.92\pm1.38\) & \(92.33\pm0.64\) & \(60.47\pm0.89\) & \(57.78\pm0.89\) \\
        Conv-6 & \(65.62\pm1.43\) & \(90.99\pm0.71\) & \(58.92\pm0.88\) & \(56.52\pm0.87\) \\
        \end{tabular}
    }
    
\end{table*}

